Hydra: an Ensemble of Convolutional Neural Networks for Geospatial Land Classification

We describe in this paper Hydra, an ensemble of convolutional neural networks (CNN) for geospatial land classification. The idea behind Hydra is to create an initial CNN that is coarsely optimized but provides a good starting pointing for further optimization, which will serve as the Hydra's body. Then, the obtained weights are fine-tuned multiple times with different augmentation techniques, crop styles, and classes weights to form an ensemble of CNNs that represent the Hydra's heads. By doing so, we prompt convergence to different endpoints, which is a desirable aspect for ensembles. With this framework, we were able to reduce the training time while maintaining the classification performance of the ensemble. We created ensembles for our experiments using two state-of-the-art CNN architectures, ResNet and DenseNet. We have demonstrated the application of our Hydra framework in two datasets, FMOW and NWPU-RESISC45, achieving results comparable to the state-of-the-art for the former and the best reported performance so far for the latter. Code and CNN models are available at https://github.com/maups/hydra-fmow

==> future_work.tex <==
%auto-ignore
\section{Future directions}

The inter-relation of land regions that are part of the same scene, as those shown in Figure~\ref{fig:contains_relations} (top), could also be exploited to improve classification. As an example, lets consider two relations \texttt{contain} and \texttt{close} as shown in Figure~\ref{fig:contains_relations} (bottom).

The \texttt{contain} relation is depicted as a unidirectional edge and is created whenever a significant portion of a region is within another region. The \texttt{close} relation is depicted as a bidirectional edge, and is used to represent the presence of two regions simultaneously in the same scene shot. The \texttt{close} relation could also have weights such as distance, e.g. obtained from the satellite metadata, to preserve the scene topology.

Then, to verify if such relations make sense in the real world we can use semantic networks such as ConceptNet~\cite{Liu2004} or geographical statistics from OpenStreetMap~\cite{4653466} and change the classifications based on this prior knowledge. Unfortunately, multiple annotations exist only for the \texttt{testing} fMoW dataset, where the ground-truth annotations are not yet public, and thus, they cannot be used evaluated neither used as training. 
\begin{figure}[!htb]
  \centering
  \begin{tikzpicture}
   \tikzset{blockA/.style={draw, ellipse, text centered, drop shadow, fill=white, text width=2.5cm, minimum height=0.55cm}}
   \tikzset{blockB/.style={draw, ellipse, text centered, drop shadow, fill=white, text width=2.1cm, minimum height=0.55cm}}
     
   \draw(2.5,7.0) node[inner sep=0pt] (image) {
      \includegraphics[width=9.0cm]{figures/image_0004691_4_rgb.jpg}   
   };
    
   \path[->](-0.3,2.0) node[blockB,inner sep=0] (box_interchange) {
      \textsc{\footnotesize Interchange}
   };
  
   \path[->](2.4,0.0) node[blockB,inner sep=0] (box_false_positive) {
      \textsc{\footnotesize False positive}
   };  
   
   \path[->](-0.3,-2.0) node[blockB,inner sep=0] (box_road_brigde) {
      \small \textsc{Road Bridge}
   };
   
   \draw [->] (box_interchange) -- (box_road_brigde) node [midway,fill=white] {Contains};
   
   %\draw [->,thick](b3)--(l2);
   
   \path[->](5.3,2.0) node[blockA,inner sep=-1] (box_amusement) {
      \textsc{\footnotesize Amusement park}
   };
   
   \path[->](5.3,-2.0) node[blockB,inner sep=0] (box_parking) {
      \small \textsc{Parking lot}
   };
   
   \draw [->] (box_amusement) -- (box_parking) node [midway,fill=white] {Contains};
   
   \draw [<->] (box_amusement) -- (box_false_positive) node [midway,fill=white] {Close};
   \draw [<->] (box_interchange) -- (box_false_positive) node [midway,fill=white] {Close};
   \draw [<->] (box_interchange) -- (box_amusement) node [midway,fill=white] {Close};
   \draw [<->] (box_road_brigde) -- (box_false_positive) node [midway,fill=white] {Close};
   \draw [<->] (box_parking) -- (box_false_positive) node [midway,fill=white] {Close};
   \draw [<->] (box_parking) -- (box_false_positive) node [midway,fill=white] {Close};
   \draw [<->] (box_parking) -- (box_road_brigde) node [midway,fill=white] {Close};   
  \end{tikzpicture} 
  \caption{Example of a fMoW image from \texttt{testing} set with eight regions, and the context relations between them.} 
  \label{fig:contains_relations}
\end{figure}   

